Minusformer: Improving Time Series Forecasting by Progressively Learning Residuals

In this paper, we find that ubiquitous time series (TS) forecasting models are prone to severe overfitting. To cope with this problem, we embrace a de-redundancy approach to progressively reinstate the intrinsic values of TS for future intervals. Specifically, we introduce a dual-stream and subtraction mechanism, which is a deep Boosting ensemble learning method. And the vanilla Transformer is renovated by reorienting the information aggregation mechanism from addition to subtraction. Then, we incorporate an auxiliary output branch into each block of the original model to construct a highway leading to the ultimate prediction. The output of subsequent modules in this branch will subtract the previously learned results, enabling the model to learn the residuals of the supervision signal, layer by layer. This designing facilitates the learning-driven implicit progressive decomposition of the input and output streams, empowering the model with heightened versatility, interpretability, and resilience against overfitting. Since all aggregations in the model are minus signs, which is called Minusformer. Extensive experiments demonstrate the proposed method outperform existing state-of-the-art methods, yielding an average performance improvement of 11.9% across various datasets.The code has been released at https://github.com/Anoise/Minusformer.

==> texes/tb3_uts_-_____.tex <==

\begin{table*}[htpb]
  \centering
  \caption{Univariate TS forecasting results on five benchmark datasets. }
  \label{tb3}
  \resizebox{0.95\textwidth}{!}
  {
    \tiny
    \begin{threeparttable}
    \begin{tabular}{cc  cc  cc  cc  cc  cc  cc  c}
      \toprule
      Model       & \multicolumn{2}{l}{Minusformer-96} & \multicolumn{2}{l}{Periodformer-144$^{\diamondsuit}$} & \multicolumn{2}{l}{FEDformer-96} & \multicolumn{2}{l}{Autoformer-96} & \multicolumn{2}{l}{Informer-96} & \multicolumn{2}{l}{LogTrans-96} & \multicolumn{2}{l}{Reformer-96} \\
      \hline
      Metric      & MSE              & MAE             & MSE               & MAE               & MSE             & MAE            & MSE             & MAE             & MSE            & MAE            & MSE            & MAE            & MSE            & MAE            \\
      \hline
      ETTh1       & {\bf\color{red}0.072}            & {\bf\color{red}0.206}           & \underline{\color{blue}0.093}             & \underline{\color{blue}0.237}             & 0.111           & 0.257          & 0.105           & 0.252           & 0.199          & 0.377          & 0.345          & 0.513          & 0.624          & 0.600          \\
      \hline
      ETTh2       & {\bf\color{red}0.185}            & {\bf\color{red}0.337}           & \underline{\color{blue}0.192}             & \underline{\color{blue}0.343}             & 0.206           & 0.350          & 0.218           & 0.364           & 0.243          & 0.400          & 0.252          & 0.408          & 3.472          & 1.283          \\
      \hline
      ETTm1       & {\bf\color{red}0.052}            & {\bf\color{red}0.172}           & \underline{\color{blue}0.059}             & \underline{\color{blue}0.201}             & 0.069           & 0.202          & 0.081           & 0.221           & 0.281          & 0.441          & 0.231          & 0.382          & 0.523          & 0.536          \\
      \hline
      ETTm2       & \underline{\color{blue}0.118}            & \underline{\color{blue}0.254}           & {\bf\color{red}0.115}             & {\bf\color{red}0.253 }            & 0.135           & 0.278          & 0.130           & 0.271           & 0.147          & 0.293          & 0.130          & 0.277          & 0.136          & 0.288          \\
      \hline
      Traffic     & {\bf\color{red}0.132}            & {\bf\color{red}0.212}           & \underline{\color{blue}0.150}             & \underline{\color{blue}0.233}             & 0.177           & 0.270          & 0.261           & 0.365           & 0.309          & 0.388          & 0.341          & 0.417          & 0.375          & 0.434          \\
      \hline
      Electricity & \underline{\color{blue}0.314}            & \underline{\color{blue}0.401}           & {\bf\color{red}0.298 }            & {\bf\color{red}0.389}             & 0.347           & 0.434          & 0.414           & 0.479           & 0.372          & 0.444          & 0.410          & 0.473          & 0.352          & 0.435          \\
      \hline
      Weather     & {\bf\color{red}0.0015}           & {\bf\color{red}0.0293}          & \underline{\color{blue}0.0017}            & \underline{\color{blue}0.0317}            & 0.008           & 0.067          & 0.0083          & 0.0700          & 0.0033         & 0.0438         & 0.0059         & 0.0563         & 0.0115         & 0.0785         \\
      \hline
      Exchange    & \underline{\color{blue}0.429}            & \underline{\color{blue}0.453}           & {\bf\color{red}0.353}             & {\bf\color{red}0.434}             & 0.499           & 0.512          & 0.578           & 0.537           & 1.511          & 1.029          & 1.350          & 0.810          & 1.028          & 0.812          \\ 
      \hline
      { $1^{\text{st}}$ Count} & {\bf\color{red} 24}           & {\bf\color{red}27}           & \underline{\color{blue}14}                   & \underline{\color{blue}12}       & 0               & 1               & 0             & 0               & 0               & 0               & 2             & 0             & 0               & 0             \\
      \bottomrule
    \end{tabular}
  \begin{tablenotes}
    \item[*] All results are averaged across all prediction lengths. The results for all prediction lengths are provided in Appendix \ref{app_uts}. ${\diamondsuit}$ denotes the maximum search range of the input length.
  \end{tablenotes}
  \end{threeparttable}
}
\end{table*}

==> texes/tb3_uts_bak.tex <==

\begin{table*}[htpb]
  \centering
  \caption{Univariate TS forecasting results on five benchmark datasets. }
  \label{tb3}
  \resizebox{0.95\textwidth}{!}
  {
    \tiny
    \begin{threeparttable}
    \begin{tabular}{cc >{\columncolor{gray!15}} cc >{\columncolor{gray!15}} cc >{\columncolor{gray!15}} cc >{\columncolor{gray!15}} cc >{\columncolor{gray!15}} cc >{\columncolor{gray!15}} cc >{\columncolor{gray!15}} c}
      \toprule
      Model       & \multicolumn{2}{l}{Minusformer-96} & \multicolumn{2}{l}{Periodformer-144$^{\diamondsuit}$} & \multicolumn{2}{l}{FEDformer-96} & \multicolumn{2}{l}{Autoformer-96} & \multicolumn{2}{l}{Informer-96} & \multicolumn{2}{l}{LogTrans-96} & \multicolumn{2}{l}{Reformer-96} \\
      \toprule
      Metric      & MSE              & MAE             & MSE               & MAE               & MSE             & MAE            & MSE             & MAE             & MSE            & MAE            & MSE            & MAE            & MSE            & MAE            \\
      \toprule
      ETTh1       & {\bf\color{red}0.072}            & {\bf\color{red}0.206}           & \underline{\color{blue}0.093}             & \underline{\color{blue}0.237}             & 0.111           & 0.257          & 0.105           & 0.252           & 0.199          & 0.377          & 0.345          & 0.513          & 0.624          & 0.600          \\
      \toprule
      ETTh2       & {\bf\color{red}0.185}            & {\bf\color{red}0.337}           & \underline{\color{blue}0.192}             & \underline{\color{blue}0.343}             & 0.206           & 0.350          & 0.218           & 0.364           & 0.243          & 0.400          & 0.252          & 0.408          & 3.472          & 1.283          \\
      \toprule
      ETTm1       & {\bf\color{red}0.052}            & {\bf\color{red}0.172}           & \underline{\color{blue}0.059}             & \underline{\color{blue}0.201}             & 0.069           & 0.202          & 0.081           & 0.221           & 0.281          & 0.441          & 0.231          & 0.382          & 0.523          & 0.536          \\
      \toprule
      ETTm2       & \underline{\color{blue}0.118}            & \underline{\color{blue}0.254}           & {\bf\color{red}0.115}             & {\bf\color{red}0.253 }            & 0.135           & 0.278          & 0.130           & 0.271           & 0.147          & 0.293          & 0.130          & 0.277          & 0.136          & 0.288          \\
      \toprule
      Traffic     & {\bf\color{red}0.132}            & {\bf\color{red}0.212}           & \underline{\color{blue}0.150}             & \underline{\color{blue}0.233}             & 0.177           & 0.270          & 0.261           & 0.365           & 0.309          & 0.388          & 0.341          & 0.417          & 0.375          & 0.434          \\
      \toprule
      Electricity & \underline{\color{blue}0.314}            & \underline{\color{blue}0.401}           & {\bf\color{red}0.298 }            & {\bf\color{red}0.389}             & 0.347           & 0.434          & 0.414           & 0.479           & 0.372          & 0.444          & 0.410          & 0.473          & 0.352          & 0.435          \\
      \toprule
      Weather     & {\bf\color{red}0.0015}           & {\bf\color{red}0.0293}          & \underline{\color{blue}0.0017}            & \underline{\color{blue}0.0317}            & 0.008           & 0.067          & 0.0083          & 0.0700          & 0.0033         & 0.0438         & 0.0059         & 0.0563         & 0.0115         & 0.0785         \\
      \toprule
      Exchange    & \underline{\color{blue}0.429}            & \underline{\color{blue}0.453}           & {\bf\color{red}0.353}             & {\bf\color{red}0.434}             & 0.499           & 0.512          & 0.578           & 0.537           & 1.511          & 1.029          & 1.350          & 0.810          & 1.028          & 0.812          \\ 
      \toprule
      { $1^{\text{st}}$ Count} & {\bf\color{red} 24}           & {\bf\color{red}27}           & \underline{\color{blue}14}                   & \underline{\color{blue}12}       & 0               & 1               & 0             & 0               & 0               & 0               & 2             & 0             & 0               & 0             \\
      \bottomrule
    \end{tabular}
  \begin{tablenotes}
    \item[*] All results are averaged across all prediction lengths. The results for all prediction lengths are provided in Appendix \ref{app_uts}. ${\diamondsuit}$ denotes the maximum search range of the input length.
  \end{tablenotes}
  \end{threeparttable}
}
\end{table*}
